The Hammock Plot: Where Categorical and Numerical Data Relax Together

Effective methods for visualizing data involving multiple variables, including categorical ones, are limited. The hammock plot (Schonlau 2003) visualizes both categorical and numerical variables using parallel coordinates. We introduce the Stata implementation hammock. We give numerous examples that explore highlighting, missing values, putting axes on the same scale, and tracing an observation across variables. Further, we discuss parallel univariate plots as an edge case of hammock plots. We also present and make publicly available a new dataset on the 2020 Tour de France.

==> stata.tex <==

\section{User's guide to stata.sty}

\texttt{stata.sty} is a {\LaTeX} package containing macros and environments to
help authors produce documents containing {\stata} output and syntax
diagrams.

\subsection{Citing the Stata manuals}

The macros for generating references to the {\stata} manuals are
given in table~\ref{table:manref}.

\clearpage
\begin{table}[h!]
\caption{Stata manual references}
\label{table:manref}
\begin{center}
\begin{tabular}{ll}
\hline
\noalign{\smallskip}
Example & Result\\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\verb+\bayesref{bayes}+ & \bayesref{bayes}\\
\verb+\cmref{cmchoiceset}+ & \cmref{cmchoiceset} \\
\verb+\dref{Data types}+ & \dref{Data types}\\
\verb+\dsgeref{dsge}+ & \dsgeref{dsge} \\
\verb+\ermref{eregress}+ & \ermref{eregress} \\
\verb+\fnref{Statistical functions}+ & \fnref{Statistical functions}\\
\verb+\fmmref{fmm:~betareg}+ & \fmmref{fmm:~betareg}\\
\verb+\grefa{Graph Editor}+ & \grefa{Graph Editor}\\
\verb+\grefb{graph}+ & \grefb{graph}\\
\verb+\grefci{line\_options}+ & \grefci{line\_options}\\
\verb+\grefdi{connectstyle}+ & \grefdi{connectstyle}\\
\verb+\gsref{6~Using the Data Editor}+ & \gsref{6~Using the Data Editor} \\
\verb+\irtref{irt}+ & \irtref{irt} \\
\verb+\lassoref{Lasso intro}+ & \lassoref{Lasso intro}\\
\verb+\metaref{meta}+ & \metaref{meta} \\
\verb+\meref{me}+ & \meref{me}\\
\verb+\mreff{Intro}+ & \mreff{Intro}\\
\verb+\mrefa{Ado}+ & \mrefa{Ado}\\
\verb+\mrefb{Declarations}+ & \mrefb{Declarations}\\
\verb+\mrefc{mata clear}+ & \mrefc{mata clear}\\
\verb+\mrefd{Matrix}+ & \mrefd{Matrix}\\
\verb+\mrefe{st\_view($\,$)}+ & \mrefe{st\_view($\,$)}\\
\verb+\mrefg{Glossary}+ & \mrefg{Glossary}\\
\verb+\miref{mi impute}+ & \miref{mi impute}\\
\verb+\mvref{cluster}+ & \mvref{cluster}\\
\verb+\pref{syntax}+ & \pref{syntax}\\
\verb+\pssrefa{Intro}+ & \pssrefa{Intro}\\
\verb+\pssrefb{power}+ & \pssrefb{power}\\
\verb+\pssrefc{ciwidth}+ & \pssrefc{ciwidth} \\
\verb+\pssrefd{Unbalanced designs}+ & \pssrefd{Unbalanced designs}\\
\verb+\pssrefe{Glossary}+ & \pssrefe{Glossary} \\
\verb+\pssref{Subject and author index}+ & \pssref{Subject and author index} \\
\verb+\rptref{Dynamic documents intro}+ & \rptref{Dynamic documents intro}\\
\verb+\rref{regress}+ & \rref{regress}\\
\verb+\spref{Intro}+ & \spref{Intro}\\
\verb+\stref{streg}+ & \stref{streg}\\
\verb+\svyref{svy:~tabulate oneway}+ & \svyref{svy:~tabulate oneway}\\
\verb+\tsref{arima}+ & \tsref{arima}\\
\verb+\uref{1~Read this---it will help}+ & \uref{1~Read this---it will help}\\
\verb+\xtref{xtreg}+ & \xtref{xtreg}\\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}

\clearpage
\subsection{Stata syntax}

Here is an example syntax display:

\begin{stsyntax}
\dunderbar{reg}ress
    \depvar\
    \optindepvars\
    \optif\
    \optin\
    \optweight\
    \optional{,
    \underbar{nocons}tant
    \underbar{h}ascons
    tsscons
    vce({\it vcetype\/})
    \underbar{l}evel(\num)
    \underbar{b}eta
    \underbar{ef}orm(\ststring)
    \dunderbar{dep}name(\varname)
    {\it display\_options}
    \underbar{nohe}ader
    \underbar{notab}le
    plus
    \underbar{ms}e1
    \underbar{coefl}egend}
\end{stsyntax}

\noindent
This syntax is generated by

\begin{stverbatim}
\begin{verbatim}
\begin{stsyntax}
\dunderbar{reg}ress
    \depvar\
    \optindepvars\
    \optif\
    \optin\
    \optweight\
    \optional{,
    \underbar{nocons}tant
    \underbar{h}ascons
    tsscons
    vce({\it vcetype\/})
    \underbar{l}evel(\num)
    \underbar{b}eta
    \underbar{ef}orm(\ststring)
    \dunderbar{dep}name(\varname)
    {\it display\_options}
    \underbar{nohe}ader
    \underbar{notab}le
    plus
    \underbar{ms}e1
    \underbar{coefl}egend}
\end{stsyntax}
\end{verbatim}
\end{stverbatim}

\noindent
Each command should be formatted using a separate \texttt{stsyntax}
environment.  Table~\ref{table:syntax} contains an example of each syntax
macro provided in \texttt{stata.sty}. 

\clearpage
\begin{table}[h!]
\caption{\stata{} syntax elements}
\label{table:syntax}
\fontsize{10}{14}\selectfont
\begin{center}
\begin{tabular}{ll@{\hspace{.5in}}ll}
\noalign{\smallskip}
\hline
\noalign{\smallskip}
Macro & Result
&
Macro & Result
\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\verb+\LB+ & \LB
&
\verb+\ifexp+ & \ifexp
\\
\noalign{\smallskip}
\verb+\RB+ & \RB
&
\verb+\optif+ & \optif
\\
\noalign{\smallskip}
\verb+\varname+ & \varname
&
\verb+\inrange+ & \inrange
\\
\noalign{\smallskip}
\verb+\optvarname+ & \optvarname
&
\verb+\optin+ & \optin
\\
\noalign{\smallskip}
\verb+\varlist+ & \varlist
&
\verb+\eqexp+ & \eqexp
\\
\noalign{\smallskip}
\verb+\optvarlist+ & \optvarlist
&
\verb+\opteqexp+ & \opteqexp
\\
\noalign{\smallskip}
\verb+\newvarname+ & \newvarname
&
\verb+\byvarlist+ & \byvarlist
\\
\noalign{\smallskip}
\verb+\optnewvarname+ & \optnewvarname
&
\verb+\optby+ & \optby
\\
\noalign{\smallskip}
\verb+\newvarlist+ & \newvarlist
&
\verb+\optional{text}+ & \optional{text}
\\
\noalign{\smallskip}
\verb+\optnewvarlist+ & \optnewvarlist
&
\verb+\optweight+ & \optweight
\\
\noalign{\smallskip}
\verb+\depvar+ & \depvar
&
\verb+\num+ & \num
\\
\noalign{\smallskip}
\verb+\optindepvars+ & \optindepvars
&
\verb+\ststring+ & \ststring
\\
\noalign{\smallskip}
\verb+\opttype+ & \opttype
\\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}

\verb+\underbar+ is a standard macro that generates underlines.  The
\verb+\dunderbar+ macro from \texttt{stata.sty} generates the underlines for
words with descenders. For example,

\begin{itemize}
\item
\verb+{\tt \underbar{reg}ress}+ generates {\tt \underbar{reg}ress}

\item
\verb+{\tt \dunderbar{reg}ress}+ generates {\tt \dunderbar{reg}ress}

\end{itemize}

The plain \TeX{} macros \verb+\it+, \verb+\sl+, and \verb+\tt+ are
also available. \verb+\it+ should be used to denote ``replaceable''
words, such as {\it varname}. \verb+\sl+ can be used for emphasis but
should not be overused. \verb+\tt+ should be used to denote words that
are to be typed, such as command names.

When describing the options of a new command, the \verb+\hangpara+ and
\verb+\morehang+ commands provide a means to reproduce a paragraph style
similar to that of the Stata reference manuals.  For example,

\hangpara
{\tt level(\num)} specifies the confidence level, as a percentage,
for confidence intervals.  The default is {\tt level(95)} or as set by {\tt
set level}; see \uref{20.8~Specifying the width of confidence intervals}.

\clearpage
\noindent
was generated by

\begin{stverbatim}
\begin{verbatim}
\hangpara
{\tt level(\num)} specifies the confidence level, as a percentage,
for confidence intervals.  The default is {\tt level(95)} or as set by {\tt
set level}; see \uref{20.8~Specifying the width of confidence intervals}.
\end{verbatim}
\end{stverbatim}


\subsection{Stata output}
\label{sec:output}

When submitting {\sl Stata Journal\/} articles that contain {\stata} output,
also submit a do-file and all relevant datasets that reproduce the output
(do not forget to set the random-number seed when doing simulations).  Results
should be reproducible. Begin examples by loading the data. Code should be
written to respect a linesize of 80 characters. The
following is an example of the \texttt{stlog} environment containing output
from simple linear regression analysis on two variables in {\tt auto.dta}:

\begin{stlog}
\input{output1.log.tex}\nullskip
\end{stlog}

\noindent
The above listing was included using

\begin{stverbatim}
\begin{verbatim}
\begin{stlog}
\input{output1.log.tex}\nullskip
\end{stlog}
\end{verbatim}
\end{stverbatim}

\noindent
where \texttt{output1.log.tex} is a Stata log file converted to include \TeX{}
macros by using the \stcmd{sjlog} command (more on \stcmd{sjlog} shortly).
\verb+\nullskip+ adjusts the spacing around the log file.

\clearpage
On occasion, it is convenient (maybe even necessary) to be able to omit some of
the output or let it spill onto the next page.  Here is a listing containing
the details of the following discussion:

\begin{stverbatim}
\begin{verbatim}
\begin{stlog}
. sysuse auto
(1978 Automobile Data)
{\smallskip}
. regress mpg weight
{\smallskip}
\oom
{\smallskip}
\clearpage
\end{stlog}
\end{verbatim}
\end{stverbatim}

The \verb+\oom+ macro creates
a short message indicating omitted output in the following example, and the
\verb+\clearpage+ macro inserts a page break.

\begin{stlog}
. sysuse auto
(1978 Automobile Data)
{\smallskip}
. regress mpg weight
{\smallskip}
\oom
{\smallskip}
\clearpage
\end{stlog}

The output in \texttt{output1.log.tex} was generated from the following
\texttt{output.do}:

\begin{stlog}
\input{output.do.log.tex}
\end{stlog}

\noindent
\texttt{output.do} generates a \stcmd{.smcl} file, \stcmd{.log} file,
and \stcmd{.log.tex} file using \stcmd{sjlog}.  The actual file used in the
above listing was generated by

\begin{stlog}
. sjlog type output.do
\end{stlog}

\texttt{sjlog.ado} is provided in the Stata package for \stcmd{sjlatex}.
\stcmd{sjlog} is a Stata command that helps generate log output to be included
in {\LaTeX} documents using the \texttt{stlog} environment.  If you have
installed the \stcmd{sjlatex} package, see the help file for \stcmd{sjlog} for
more details.  The lines that make up the table output from \stcmd{regress}
are generated from line-drawing macros defined in \texttt{stata.sty}; these
were macros written using some font metrics defined in \citet{texbook}.

By default, \texttt{stlog} sets an 8-point font for the log.  Use the
\texttt{auto} option to turn this behavior off, allowing you to use the
current font size, or change it by using\\ \verb+\fontsize{#}{#}\selectfont+.
The call to \texttt{stlog} with the \texttt{auto} option looks like
\verb+\begin[auto]{stlog}+.

Here is an example where we are using a 12-point font.

\vspace{-.2in}
{\fontsize{12}{13}\selectfont
\begin{stlog}[auto]
. sjlog type output.do
\end{stlog}
}

\subsection{About tables}

Tables should be created using the standard \LaTeX{} methods.  See
\citet{latexbook} for a discussion and examples. Tables should be included in
the main text rather than at the end of the document. Tables should be called
out in the text prior to appearance.

\clearpage
There are many user-written commands that produce \LaTeX{} output, including
tables.  Christopher F. Baum has written \stcmd{outtable}, a Stata command for
creating \LaTeX{} tables from Stata matrices.  Ben Jann's well-known
\stcmd{estout} command can also produce \LaTeX{} output.  To find other
user-written commands that produce \LaTeX{} output, try

\begin{stlog}
. net search latex
\end{stlog}

\subsubsection{Tables with notes}

Table~\ref{Table4} shows the order and format to use for notes to tables.

\begin{table}[h!]
\begin{threeparttable}
\centering
\caption{Industrial clusters}
\label{Table4}
\begin{tabularx}{\textwidth}{X  p{1.5cm}  p{1pt}  X  p{1.5cm}}
\hline
\multicolumn{2}{c}{China} & & \multicolumn{2}{c}{United States} \\
\cline{1-2} \cline{4-5}
Core of cluster & Size (in $\num$ of units) & & Core of cluster & Size (in $\num$ of units) \\
\cline{1-2} \cline{4-5}
Construction & 28$^{\rm a}$ & & Public administration and defense; compulsory social
security & 30$^{\rm b}$ \\
Food, beverages, and tobacco & 3 & & Food, beverages, and tobacco & 2 \\
Textiles and textile products & 2 & & Chemicals and chemical products & 1 \\
Chemicals and chemical products & 1 & & Basic metals and fabricated metal & 1 \\
Transport equipment & 1 & & Transport equipment & 1 \\
\hline
\multicolumn{2}{l}{$L_a=0.602$***} & & \multicolumn{2}{l}{$L_a=0.567$} \\
\multicolumn{2}{l}{$L_w=0.828$**} & & \multicolumn{2}{l}{$L_w=0.837$} \\
\multicolumn{2}{l}{$L_m=0.335$*} & & \multicolumn{2}{l}{$L_m=0.287$} \\
\multicolumn{2}{l}{$K^*=5$} & & \multicolumn{2}{l}{$K^*=5$} \\
\multicolumn{2}{l}{$K=35$} & & \multicolumn{2}{l}{$K=35$} \\
\hline
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item \textsc{source:} Pew Research Center.
\item \textsc{note:} U.S.~industrial clusters based on
U.S.~input--output flows of goods expressed in millions of dollars between 35
{\smrm ISIC} industries from the {\smrm WIOD} data. The minimum number of
clusters \texttt{k()} was set equal to five. The algorithm returns $L_a$,
$L_w$, and $L_m$, which refer to the average of the internal relative
flows, the population-weighted average of the internal relative
flows, and the minimum of the internal relative flows,
respectively. $K^*$ and $K$ refer to the number of defined regional clusters
and the number of distinct starting units, respectively.
\item $^{\rm a}$ This note pertains only to row 1 column 2.
\item $^{\rm b}$ This note pertains only to row 1 column 4.
\item *** denotes $p<0.01$; ** denotes $p<0.05$; * denotes $p<0.1$.
\end{tablenotes}
\end{threeparttable}
\end{table}

Order of notes should be
\vspace{-.08in}
\begin{enumerate}
\item source notes
\item notes applying to the whole table
\item notes applying to specific parts of the table
\item notes on significance levels
\end{enumerate}

Special notes:

\vspace{-.08in}
\begin{itemize}
\item Use \verb+\centering+ because the {\tt center} environment adds
unnecessary vertical spacing.

\item Place the \verb+\begin{threeparttable}+ line above the caption.

\end{itemize}

Tables should be included in the main text rather than at the end of the
document. Tables should be called out in the text prior to appearance.

\subsection{Encapsulated PostScript (EPS)}

You can include figures by using either \verb+\includegraphics+ or
\verb+\epsfig+.

\begin{stverbatim}
\begin{verbatim}
\begin{figure}[h!]
\begin{center}
\includegraphics{eps/output1.eps}
\end{center}
\caption{Scatterplot with simple linear regression line}
\label{fig}
\end{figure}
\end{verbatim}
\end{stverbatim}

\begin{stverbatim}
\begin{verbatim}
\begin{figure}[h!]
\begin{center}
\epsfig{file=output1}
\end{center}
\caption{Scatterplot with simple linear regression line}
\label{fig}
\end{figure}
\end{verbatim}
\end{stverbatim}

Figure~\ref{fig} is included using \verb+\epsfig+ from the \texttt{epsfig}
package.  

\noindent
The graph was generated by running \texttt{output.do}, the
do-file given in section~\ref{sec:output}.  The \texttt{epsfig} package is
described in \citet*{latexcompanion}.

\clearpage

\begin{figure}[h!]
\begin{center}
\epsfig{file=output1}
\end{center}
\caption{Scatterplot with simple linear regression line}
\label{fig}
\end{figure}

{\smrm EPS} is the preferred format for graphs and line art. Figures should be
included in the main text rather than at the end of the document and should be
called out in the text prior to appearance. If your article is written in
Word, you should submit your figures as separate {\smrm EPS} files. Rasterized-based
files of at least 300 dpi (dots per inch) are acceptable. Avoid using bitmaps
for figures and graphs, because even if images are outputted at 300 dpi,
bitmaps can increase the size of the resulting file for printing. (However,
bitmaps will be allowed for photographs, which are used in, for example, the
{\sl Stata Journal} Editors' prize announcement.) Images should be submitted in
black and white (grayscale). We recommend that graphs created in Stata use the
{\tt sj} scheme.

\subsection{Stored results}

The \texttt{stresults} environment provides a table to describe the stored
results of a Stata command.  It consists of four columns: the first and third
column are for Stata result identifiers (for example, \stcmd{r(N)},
\stcmd{e(cmd)}), and the second and fourth columns are for a brief description
of the respective identifier.
%
Each group of results is generated using the \verb+\stresultsgroup+ macro.
%
The following is an example containing a brief description of the results that
\stcmd{regress} stored to \stcmd{e()}:

\clearpage

\begin{stresults}
\stresultsgroup{Scalars} \\
\stcmd{e(N)} & number of observations
&
\stcmd{e(F)} & $\scriptstyle F$ statistic
\\
\stcmd{e(mss)} & model sum of squares
&
\stcmd{e(rmse)} & root mean squared error
\\
\stcmd{e(df\_m)} & model degrees of freedom
&
\stcmd{e(ll\_r)} & log likelihood
\\
\stcmd{e(rss)} & residual sum of squares
&
\stcmd{e(ll\_r0)} & log likelihood, constant-only\\
\stcmd{e(df\_r)} & residual degrees of freedom
&
& \quad model \\
\stcmd{e(r2)} & $\scriptstyle R$-squared
&
\stcmd{e(N\_clust)} & number of clusters
\\
\stresultsgroup{Macros} \\
\stcmd{e(cmd)} & \stcmd{regress}
&
\stcmd{e(wexp)} & weight expression
\\
\stcmd{e(depvar)} & name of dependent variable
&
\stcmd{e(clustvar)} & name of cluster variable
\\
\stcmd{e(model)} & \stcmd{ols} or \stcmd{iv}
&
\stcmd{e(vcetype)} & title used to label Std.~Err.
\\
\stcmd{e(wtype)} & weight type
&
\stcmd{e(predict)} & program used to implement
\\
&&&\quad \stcmd{predict}
\\
\stresultsgroup{Matrices} \\
\stcmd{e(b)} & coefficient vector
&
\stcmd{e(V)} & variance--covariance matrix of
\\
&&&\quad the estimators\\
\stresultsgroup{Functions} \\
\stcmd{e(sample)} & marks estimation sample
\\
\end{stresults}

Alternatively, you can use the \texttt{stresults2} environment to create
a two column table.   This format works better if your descriptions are long.

\subsection{Examples and notes}

The following are environments for examples and notes similar to those
given in the Stata reference manuals.  They are generated using the
\texttt{stexample} and \texttt{sttech} environments, respectively.


\begin{stexample}
This is the default alignment for a \stata{} example.
\end{stexample}

\setlength{\stexamplehskip}{0pt}
\begin{stexample}
For this example, \verb+\stexamplehskip+ was set to
\texttt{\the\stexamplehskip}
before beginning.  This sentence is supposed to spill
over to the next line, thus revealing that the first sentence was indented.

This sentence is supposed to show that new paragraphs are automatically
indented (provided that \verb+\parindent+ is nonzero).
\end{stexample}

\clearpage
\begin{sttech}
For this note, \verb+\sttechhskip+ was set to \texttt{\the\sttechhskip}
(the default) before beginning.  This sentence is supposed to spill over to
the next line, thus revealing that the first sentence was indented.

This sentence is supposed to show that new paragraphs are automatically
indented (provided that \verb+\parindent+ is nonzero).
\end{sttech}

\subsection{Special characters}

Table \ref{table:specialch} contains macros that generate some useful
characters in the typewriter (fixed width) font.  The exceptions are
\verb+\stcaret+ and \verb+\sttilde+, which use the currently specified font;
the strictly fixed-width versions are \verb+\caret+ and \verb+\tytilde+,
respectively.

\begin{table}[h!]
\caption{Special characters}
\label{table:specialch}
\begin{center}
\begin{tabular}{ll@{\hspace{.5in}}ll}
\hline
\noalign{\smallskip}
Macro & Result &
Macro & Result \\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\verb+\stbackslash+ & \stbackslash
 &
\verb+\sttilde+ & \sttilde
\\
\verb+\stforslash+ & \stforslash 
&
\verb+\tytilde+ & \tytilde
\\
\verb+\stcaret+ & \stcaret
&
\verb+\lbr+ & \lbr
\\
\verb+\caret+ & \caret
&
\verb+\rbr+ & \rbr
\\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}


\subsection{Equations and formulas}

In (\ref{eq:Exbar}), $\stbar{x}$ was generated using
\verb+\stbar{x}+.  Here \verb+\stbar+ is equivalent to the \TeX{} macro
\verb+\overline+.

\begin{equation}
E(\stbar{x}) = \mu
\label{eq:Exbar}
\end{equation}

In (\ref{eq:varbetahat}), $\sthat{\beta}$ was generated using
\verb+\sthat{\beta}+.  Here \verb+\sthat+ is equivalent to the \TeX{} macro
\verb+\widehat+.

\begin{equation}
V(\sthat{\beta}) = V\{(X'X)^{-1}X'y\} = (X'X)^{-1}X'V(y)X(X'X)^{-1}
\label{eq:varbetahat}
\end{equation}

\clearpage

Formulas should be defined and follow a concise style. Different
disciplines adhere to different notation styles; however, if the
notation cannot be clearly interpreted, you may be asked to make
changes. The bolding and font selection guidelines are the following:

\begin{itemize}
\item
	Matrices are capitalized and bolded; for instance, $\boldsymbol\Pi +
	\boldsymbol\Theta + \boldsymbol\Phi - \mathbf{B}$.

\item
	Vectors are lowercased and bolded; for instance, $\boldsymbol\pi +
	\boldsymbol\theta + \boldsymbol\phi - \mathbf{b}$.

\item
        Scalars are lowercased and nonbolded; for instance, $r_2 + c_1 - c_2$.
\end{itemize}


Sentence punctuation should not be used in formulas set off from the text.

Formulas in line with the text should use the solidus (/) instead of a
horizontal line for fractional terms.

Nesting of grouping is square brackets, curly braces, and then parentheses, or
[\{()\}].

Only those equations explicitly referred to in the text should be assigned an
equation number.

%\subsection{Other miscellaneous macros and environments}
%
%The following box was created by
%
%\begin{stverbatim}
%\begin{verbatim}
%\fbox{
%A special framed
%box that obeys lines and spaces.
%}
%\end{verbatim}
%\end{stverbatim}
%
%\fbox{
%A special framed
%box that obeys lines and spaces.
%}
%
%The following box was created by
%
%\begin{stverbatim}
%\begin{verbatim}
%\fbox{
%Test that the width of the
%box is \the\ttboxWd
%and is indented \the\ttboxIndent
%}
%\end{verbatim}
%\end{stverbatim}
%
%\fbox{
%Test that the width of the
%box is \the\ttboxWd
%and is indented \the\ttboxIndent
%}
%
\endinput


==> stata_output/auto_order_low.log.tex <==
. hammock mpg headroom price rep78 weight foreign , ///
>  missing ///
>  label_format(\%8.0g) ///
>  yline(8) /// 
>  colorlist(dkgreen\%20)

